Distributed model predictive control for continuous-time nonlinear systems based on suboptimal ADMM

The paper presents a distributed model predictive control (DMPC) scheme for continuous-time nonlinear systems based on the alternating direction method of multipliers (ADMM). A stopping criterion in the ADMM algorithm limits the iterations and therefore the required communication effort during the distributed MPC solution at the expense of a suboptimal solution. Stability results are presented for the suboptimal DMPC scheme under two different ADMM convergence assumptions. In particular, it is shown that the required iterations in each ADMM step are bounded, which is also confirmed in simulation studies.

==> figs/tikz/SysDescrCMPC.tex <==
\section{System description and centralized MPC properties}
%==========================================================================================%
\label{sec:problem_statement}


The DMPC scheme in this paper is presented for nonlinear
continuous-time systems, where the subsystems are coupled via their
state variables. This section presents the problem statement along
with the considered MPC formulation and summarizes the stability
properties in a centralized MPC setting that serve as the basis for
the subsequent DMPC scheme in the following sections.






\subsection{Problem formulation}
%------------------------------------------------------------------------------------------%

Distributed systems consisting of coupled dynamical systems are
conveniently described by a directed graph $ \mathcal{G} = ( \Vcal, \mathcal{E} ) $, 
where the nodes $i\in \Vcal =\{1, \dots, N\}$ represent the dynamical
subsystems and the edges $\mathcal{E} \subseteq \Vcal \times \Vcal$
reflect the coupling between two subsystems.
%
The dynamics of subsystem $i\in\Vcal$ is described by
%
\begin{equation}\label{eq:dyn_subsys}
  \dot{\xsys}_i = f_i ( \xsys_i, \usys_i, [\xsys_j]_{j\in\Ngets{i}} )
\end{equation}
%
with the state $\xsys_i \in \Rbb^{n_i}$ and control $\usys_i \in
\Rbb^{m_i}$. 
The coupling to neighboring subsystems is given by the states $\xsys_j$ 
using the stacking notation
$[\xsys_j]_{j\in\Ngets{i}}\in\Rbb^{p_i}$ with 
$p_i := \sum_{ j \in \Ngets{i}} n_j$ and $p=\sum_{i\in\Vcal} p_i$, whereby 
$\Ngets{i} = \{j: (j,i) \in \mathcal{E}, j \not=i \}$. 
Vice versa, $\Nto{i} = \{j: (i,j) \in \mathcal{E}, j \not= i \}  $
represent the neighbors that subsystem $i\in\Vcal$ influences.
In view of a distributed control scheme, $\Ngets{i}$ represent the 
``sending'' neighbors, whereas $\Ngets{i}$ denote the ``receiving''
neighbors. 

%
\begin{figure}
	\centering
	{
		\normalsize
		\resizebox{0.3\textwidth}{!}{\import{}{coupling.pdf_tex}}}
	\caption{Coupling structure for example system~\eqref{eq:DMPC_simple_example}.}
	\label{fig:couplStrucure}
\end{figure}
%

Figure~\ref{fig:couplStrucure} shows an example of a 
coupled system with the dynamics
%
\begin{align} \nonumber
\dot \xsys_1 &= f_1(\xsys_1,\usys_1,\xsys_2)
\\ \label{eq:DMPC_simple_example}
\dot \xsys_2 &= f_2(\xsys_2,\usys_2,\xsys_1,\xsys_3)
\\ \nonumber
\dot \xsys_3 &= f_3(\xsys_3,\usys_3,\xsys_1) \,.
\end{align}
%
The directed graph is defined by the knots $\Vcal=\{1,2,3\}$ and 
edges $\mathcal{E}=\{(1,2),(1,3),(2,1),(3,2)\}$.
The sending and receiving neighborhoods are 
$\Ngets{1}=\{2\}$, $\Ngets{2}=\{1,3\}$, $\Ngets{3}=\{1\}$ and 
$\Nto{1}=\{1,3\}$, $\Nto{2}=\{1\}$, $\Ngets{3}=\{2\}$, respectively.



The coupled subsystems~\eqref{eq:dyn_subsys} can be equivalently written in the
centralized form
%
\begin{equation}
\label{eq:dyn_sys}
\dot{\xsys}  = F (\xsys,\usys)
\end{equation}
%
with $F=[f_i]_{i\in\Vcal}$ and the stacked state and control vectors 
$\xsys = [ \xsys_i ]_{ i \in \Vcal }\in\Rbb^{n}$, 
$\usys = [ \usys_i ]_{ i \in \Vcal } \in \Rbb^{m}$ 
of dimension $ n := \sum_{i \in \Vcal} n_i$ and $m := \sum_{i \in \Vcal} m_i $,
respectively.
Without loss of generality, the control task consists in controlling
each subsystem \eqref{eq:dyn_subsys} to the origin, i.e.\
$0=f_i(0,0,0)$, $i\in\Vcal$ or equivalently $0=F(0,0)$ in the
centralized form~\eqref{eq:dyn_sys}. 

The MPC scheme to be considered is based on the online solution of the
optimal control problem (OCP) 
%
\begin{subequations}\label{eq:gl_ocp_in_gl_quant}
  \begin{align} \label{eq:gl_ocp_in_gl_quant_cost}
    \mymin\limits_{\umpc} \quad & J(\umpc,\xsys_k) := V( \xmpc(T) ) + \int_{0}^{T} { l ( \xmpc(\tau), \umpc(\tau) ) \dd \tau } \\
    % ....................................................................................
    \subjto  \quad & \dot{\xmpc}  = F (\xmpc,\umpc)\,, \quad \xmpc(0) = \xsys_k\\
    \label{eq:gl_ocp_in_gl_quant_constr}
    & \umpc \in U \text{,}
  \end{align}
%
where the cost functional \eqref{eq:gl_ocp_in_gl_quant_cost} with the
horizon length $T>0$ consists
of the integral and terminal cost functions for the single subsystems,
i.e.\
%
\begin{equation}
\label{eq:gl_ocp_in_gl_quant_cost_sum}
V(\xmpc) := \sum_{i\in \Vcal} V_i(\xmpc_i)\,, \quad
l(\xmpc,\umpc) := \sum_{i\in \Vcal} l_i(\xmpc_i,\umpc_i)
\end{equation}
\end{subequations}
%
with $l_i:\Rbb^n \times \Rbb^m \to \Rbb_0^+ $ and $V_i: \Rbb^n \to \Rbb_0^+$,
respectively. 
The set $U$ is the Cartesian product $\prod_{i\in\Vcal}U_i$ of the
compact and convex constraint sets $U_i$ for the controls $u_i$ of
the subsystems \eqref{eq:dyn_subsys}.
The initial value $\xsys(t_k) = \xsys_k = [ \xsys_{k,i} ]_{i \in \Vcal}$ is the
current (measured or observed) state of the system~\eqref{eq:dyn_subsys} at
sampling instant $t_k$.
%
The optimal solution of \eqref{eq:gl_ocp_in_gl_quant} is denoted by
$\xmpc^*(\tau;\xsys_k)$ and $\umpc^*(\tau;\xsys_k)$, $\tau\in[0,T]$
with the optimal (minimal) cost 
%
\begin{equation}
\label{eq:Jopt}
J^*(\xsys_k):=J(\umpc^*(\cdot;\xsys_k),\xsys_k)\,.
\end{equation}
%
As ususally done in MPC, the first part of the control trajectory
is applied to each subsystem~\eqref{eq:dyn_subsys} on the current sampling
interval
%
\begin{equation}
\label{eq:optcon:contrlaw}
\usys_i(t_k+\tau) = \umpc_i^*(\tau;\xsys_k) 
%=: \kappa_i^*(x^*(\tau;\ubar x_k);\ubar x_k)
\,, \quad \tau\in[0,\dt)\,, \quad i\in\Vcal
\end{equation}
%
with the sampling time $\Delta t>0$.
From the centralized viewpoint and by the principle of optimality, the
optimal control can be interpreted as a nonlinear control law of the form 
%
\begin{equation}
\label{eq:optcontrlaw_centralized}
\umpc^*(\tau;\xsys_k) =:\kappa^*(\xmpc^*(\tau;\xsys_k);\xsys_k) \,,
\quad
\tau\in[0,\Delta t)\,.
\end{equation}

The integral and terminal cost functions in~\eqref{eq:gl_ocp_in_gl_quant_cost_sum}
are typically designed in quadratic form. In particular, it is assumed that there
exist constants $m_l,M_l>0$ and $m_V,M_V\ge 0$ such that the
centralized cost functions satisfy
%
\begin{equation}
  \label{eq:bounds_cost}\arraycolsep1mm
  \begin{array}{rcl}
    m_l  (\norm x ^2 + \norm u ^2) \leq & l(x,u) &\leq M_l ( \norm x ^2 + \norm u ^2 ) \\
    m_V \norm x ^2 \leq & V(x) &\leq M_V \norm x ^2 \text{.}
  \end{array}
\end{equation}
%
The dynamics function \eqref{eq:dyn_subsys}, resp.\
\eqref{eq:dyn_sys}, and the cost functions
\eqref{eq:gl_ocp_in_gl_quant_cost_sum} are supposed to be  
continuously differentiable. Moreover, throughout the paper, it is
assumed that every bounded control
trajectory $u(t)\in U$, $t\in[0,T]$ yields a bounded state response 
$x(t)$, $t\in[0,T]$ and that
an optimal solution of \eqref{eq:gl_ocp_in_gl_quant} exists.



\subsection{Centralized MPC}
%------------------------------------------------------------------------------------------%
\label{sec:MPC_centralized}



The MPC scheme is based on an OCP
formulation~\eqref{eq:gl_ocp_in_gl_quant} without terminal
constraints, which is motivated from the practical viewpoint to
reduce the computational burden in an actual implementation. This
section summarizes stability results from the literature on MPC without
terminal constraints~\cite{Limon:TAC:2006,Graichen:TAC:2010,Graichen:INTECH:2012}.
These results also serve as the basis for investigating the stability
properties of the DMPC scheme developed in the next sections.

Several assumptions are necessary at this point.
A common assumption in MPC is that the terminal cost $V(x)$ is
designed as a control Lyapunov function (CLF) detailed as follows. 



\begin{assumption}
  \label{as:clf_on_omega}
  There exists a feedback law 
  $ u = \kappa_V (x) \in U $ 
  and a non-empty compact set 
  $ \Omega_{\beta}= \left\{ x \in \Rbb^n: V(x) \leq \beta \right\}$ 
  such that 
  $ \dot{V} ( x, \kappa_V(x) ) +  l ( x, \kappa_V(x) ) \leq 0$ $\forall x \in \Omega_{\beta}$ 
  with $ \dot{V} := (\partial V / \partial x ) F $.
\end{assumption}

Provided that the linearization of the system~\eqref{eq:dyn_sys} about the origin is
stabilizable, the terminal cost $V(x)$ and a linear feedback law
$\kappa_V(x)$ can be computed by solving a Riccati or Lyapunov
equation, which stabilizes the nonlinear system on a (possibly small)
set $\Omega_\beta$~\cite{Michalska:TAC:1993,Parisini:AUT:1995,Chen:AUT:1998}.


%
\begin{lemma} \label{lem:MPC:xT}
  Suppose that Assumption \ref{as:clf_on_omega} holds and consider the set 
  %
  \begin{equation}
    %\label{eq:levelsetdef}
    \label{eq:levelsetalpha}
    \Gamma_\alpha = \left\{x \in \Rbb^n \,|\, J^*(x) \leq \alpha
    \right\}\,, \quad
    \alpha = \beta \left( 1 + \frac{m_l}{M_V}T \right)\,.
  \end{equation}
  %
  Then, $\xmpc^*(T;\xsys_k)\in\Omega_\beta$ and $\Omega_\beta\subseteq\Gamma_\alpha$.
\end{lemma}

Lemma~\ref{lem:MPC:xT} states that the end point of the optimal
trajectory $\xmpc^*(T;\xsys_k)$ automatically lies inside the region
$\Omega_\beta$ of the CLF terminal cost. Moreover, $\Gamma_\alpha$
contains the region $\Omega_\beta$ and can be enlarged by increasing
$T$ as indicated by \eqref{eq:levelsetalpha}.
The proof of Lemma~\ref{lem:MPC:xT} can be found in
\cite{Graichen:INTECH:2012}. 



This result eventually leads to the following
Theorem~\ref{theo:exp_stab_centr_MPC} concerning the stability 
of the centralized MPC scheme over the domain of attraction
$\Gamma_\alpha$. 


\begin{theorem}  \label{theo:exp_stab_centr_MPC}
  Suppose that Assumption~\ref{as:clf_on_omega} holds. Then, 
  %with $\alpha$ according to \eqref{eq:levelsetalpha},
  %
  \begin{equation}
    \label{eq:cost_decrease_centr_MPC_terminal_cost}
    J^*(\xmpc^*(\dt,\xsys_k)) \le J^*(\xsys_k) - \int_0^{\dt}
    l(\xmpc^*(\tau;\xsys_k),\umpc^*(\tau;\xsys_k)) \dd\tau \quad
    \forall\xsys_k \in \Gamma_\alpha
  \end{equation}
  % 
  and the centralized MPC scheme 
  stabilizes the origin in the sense of 
  $\mylim_{t\to\infty}\|\xsys(t)\|=0$ for all
  $\xsys(0)=\xsys_0 \in \Gamma_\alpha$.
\end{theorem}

Theorem~\ref{theo:exp_stab_centr_MPC} (and the corresponding proof) is
a simplified version of the one given in \cite{Graichen:TAC:2010}. The
stability in the sense of $\mylim_{t\to\infty}\|\xsys(t)\|=0$ follows
from standard arguments in MPC using Barbalat's lemma. Stronger
results such as exponential stability require additional continuity
assumptions that will be employed later on in the paper. 



